Branch and Cut for Partitioning a Graph into a Cycle of Clusters

In this paper we study formulations and algorithms for the cycle clustering problem, a partitioning problem over the vertex set of a directed graph with nonnegative arc weights that is used to identify cyclic behavior in simulation data generated from nonreversible Markov state models. Here, in addition to partitioning the vertices into a set of coherent clusters, the resulting clusters must be ordered into a cycle such as to maximize the total net flow in the forward direction of the cycle. We provide a problem-specific binary programming formulation and compare it to a formulation based on the reformulation-linearization technique (RLT). We present theoretical results on the polytope associated with our custom formulation and develop primal heuristics and separation routines for both formulations. In computational experiments on simulation data from biology we find that branch and cut based on the problem-specific formulation outperforms the one based on RLT.

==> Defines.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%
% Latex Defines		%
% @author Leon Eifler	%
% @email eifler@zib.de	%
%&&&&&&&&&&&&&&&&&&&&&&&&

%% \usepackage{todonotes,xspace}
%% \newcommand{\AG}[2][]{\todo[color=green!20!yellow,#1,size=tiny]{AG: #2}}
%% \newcommand{\AGil}[1]{\AG[inline]{#1}}
%% \newcommand{\LE}[2][]{\todo[color=yellow!80!blue!20,#1,size=tiny]{LE: #2}}
%% \newcommand{\LEil}[1]{\LE[inline]{#1}}
%% \setlength{\marginparwidth}{4.2cm}

\newcommand{\ourparagraph}[1]{\medskip \noindent\textit{#1}.}

\usepackage{amsmath}
\usepackage{amssymb}
\usepackage{bbm}
\usepackage{textgreek}
\usepackage{mathtools}
\usepackage{calc}
\usepackage{xspace}
\usepackage{xcolor}
\usepackage{booktabs}
\usepackage{multirow}
\usepackage{collcell}
\usepackage{tikz}
\usepackage{tikzscale}
\usepackage{pgfplots}
\pgfplotsset{compat=1.9}
%\usepackage{subcaption}

%\usepackage{rotating}
%\usepackage{pdflscape}
%\usepackage{longtable}
%\usepackage{todonotes}
%\usepackage{amsthm}
%\usepackage{amsmath}
%\usepackage{color}
%\usepackage{graphicx}

%% % environments
%% \newtheorem{Def}{Definition}
%% \newtheorem{Lem}[Def]{Lemma}
%% \newtheorem{Rem}[Def]{Remark}
%% \newtheorem{Thm}[Def]{Theorem}
%% \newtheorem{Obs}[Def]{Observation}
%% \newtheorem{Cor}[Def]{Corollary}

% general shortcuts
\newcommand{\st}{s.t.\xspace}
\newcommand{\ie}{i.e.,\xspace}
\newcommand{\eg}{e.g.,\xspace}
\newcommand{\cf}{cf.\xspace}
\newcommand{\Wlog}{W.l.o.g.\ }


% branch-and-bound
\newcommand{\bandb}{branch-and-bound\xspace}
\newcommand{\Bandb}{Branch-and-bound\xspace}
\newcommand{\BandB}{Branch-and-Bound\xspace}

% mathematical notation
\newcommand{\NP}{\mathcal{NP}}

\newcommand{\Abs}[1]{\vert #1\vert}
\newcommand{\Norm}[1]{\Vert #1\Vert}
\newcommand{\intvars}{\mathcal{I}}
\newcommand{\allvars}{\mathcal{N}}
\newcommand{\binvars}{\mathcal{B}}
\newcommand{\trick}{switch-trick}

\newcommand{\Conv}[1]{\mathcal{#1}}
\newcommand{\optMIP}[1]{#1^{\star}}
\newcommand{\optLP}[1]{#1^{\star}_{LP}}

\newcommand{\floor}[1]{\lfloor #1\rfloor}
\newcommand{\ceil}[1]{\lceil #1\rceil}

\newcommand{\fa}{\text{for all }}
\newcommand{\cardi}[1]{|#1|}

\DeclareMathOperator{\diag}{diag}

\pgfplotsset{
	/pgf/number format/textnumber/.style={
		fixed,
		fixed zerofill,
		precision=2,
		1000 sep={.},
	},
}
\newcommand{\ApplyColor}[1]{%
	 \ifdim #1pt<0.95pt \textcolor{blue}{#1}\else
	\ifdim #1pt>1.05pt \textcolor{red}{#1}\else #1 \fi
	\fi
}


\newcolumntype{R}{>{\collectcell\ApplyColor}{r}<{\endcollectcell}}

% numbers
\newcommand{\N}{\mathbb{N}\xspace}
\newcommand{\B}{\mathbb{B}\xspace}
\newcommand{\Z}{\mathbb{Z}\xspace}
\newcommand{\R}{\mathbb{R}\xspace}
\newcommand{\1}{\mathbb{1}\xspace}

%\newcommand{\TransMat}{P\xspace}
\newcommand{\Bins}{V\xspace}
\newcommand{\NetFlow}{f}
\newcommand{\Coherence}{g}
\newcommand{\Cluster}{\mathcal{K}\xspace}
\newcommand{\Clusters}{\mathcal{C}\xspace}
\newcommand{\clustind}{\kappa}
\newcommand{\Edges}{E\xspace}
\newcommand{\Trans}{A\xspace}
\newcommand{\copen}[1]{c_{#1}\xspace}
\newcommand{\coh}{\Coherence\xspace}
\newcommand{\flow}{\NetFlow\xspace}
\DeclareMathOperator{\der}{d}
\newcommand{\percentage}[2]{\pgfmathparse{(1 - #1/#2) *100}\pgfmathprintnumber[precision=1]{\pgfmathresult}\%}
\newcommand{\reduction}[2]{\pgfmathparse{(#1)/#2 }{\pgfmathprintnumber[textnumber]{\pgfmathresult}}}
\newcommand{\boldblue}[1]{\textcolor{blue}{$\mathbf{#1}$}}
\newcommand{\boldred}[1]{\textcolor{red}{$\mathbf{#1}$}}

\newcommand{\colorquot}[2]{
	\pgfmathparse{(#1<0.9*#2)?1:0}\ifdim\pgfmathresult pt>0pt \textcolor{blue}{$\mathbf{\reduction{#1}{#2}}$}\else
	\pgfmathparse{(#1>1.1*#2)?1:0}\ifdim\pgfmathresult pt>0pt \textcolor{red}{$\mathbf{\reduction{#1}{#2}}$} \else 
	$\reduction{#1}{#2}$\fi \fi
}
\newcommand{\primdugap}[2]{\pgfmathparse{(#2-#1)/#1 *100}\pgfmathprintnumber[precision=1]{\pgfmathresult}\%}
\newcommand{\quotient}[2]{\pgfmathparse{(#1)/#2 }\pgfmathprintnumber[precision=2]{\pgfmathresult}}


%pseudo code
\usepackage{algorithm}
\usepackage{algpseudocode}
\renewcommand{\algorithmicrequire}{\textbf{Input:}}
\renewcommand{\algorithmicensure}{\textbf{Output:}}

\DeclareMathOperator*{\argmin}{arg\,min\,}
\DeclareMathOperator*{\argmax}{arg\,max\,}
\DeclareMathOperator{\conv}{conv}

\DeclareMathOperator{\spn}{span}
\DeclareMathOperator{\aff}{aff}
\newcommand*{\Signature}[1]{%
	\par\noindent\makebox[2.5in]{\hrulefill} 
	\par\noindent\makebox[2.5in][l]{#1}      
}%

\usepackage{enumitem}
%\newdateformat{myformat}{\THEDAY{. }\monthname[\THEMONTH], \THEYEAR}
\usepackage{array}
\newcolumntype{$}{>{\global\let\currentrowstyle\relax}}
\newcolumntype{^}{>{\currentrowstyle}}
\newcommand{\rowstyle}[1]{\gdef\currentrowstyle{#1}%
	#1\ignorespaces
}


